Domain Specific Language for Geometric Relations between Rigid Bodies targeted to robotic applications

This paper presents a DSL for geometric relations between rigid bodies such as relative position, orientation, pose, linear velocity, angular velocity, and twist. The DSL is the formal model of the recently proposed semantics for the standardization of geometric relations between rigid bodies, referred to as `geometric semantics'. This semantics explicitly states the coordinate-invariant properties and operations, and, more importantly, all the choices that are made in coordinate representations of these geometric relations. This results in a set of concrete suggestions for standardizing terminology and notation, allowing programmers to write fully unambiguous software interfaces, including automatic checks for semantic correctness of all geometric operations on rigid-body coordinate representations. The DSL is implemented in two different ways: an external DSL in Xcore and an internal DSL in Prolog. Besides defining a grammar and operations, the DSL also implements constraints. In the Xcore model, the Object Constraint Language language is used, while in the Prolog model, the constraint are natively modelled in Prolog. This paper discusses the implemented DSL and the tools developed on top of this DSL. In particular an editor, checking the semantic constraints and providing semantic meaningful errors during editing is proposed.

==> macroCoordinateRepresentations.tex <==
% \input{macroSemantics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% POSITION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% position vector: from point #1 belonging to body #2 to point #3 belonging to body #4, expressed in orientation frame #5
\newcommand{\posvec}[5]
 {\vphantom{p}_{\orientation{#5}}
 {\hspace*{-0.1ex}\boldsymbol{p}^{\point{#1} \ifthenelse{\equal{#2}{}}{}{|\body{#2}}, \point{#3} \ifthenelse{\equal{#4}{}}{}{|\body{#4}}}}\vphantom{p}
 }
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ORIENTATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%  \newcommand{\rot}[4]%
%   {\vphantom{R}_{\orientation{#3}\ifthenelse{\equal{#4}{}}{}{
%   \ifthenelse{\equal{#3}{}}{}{|}
%   \body{#4}}}^{\hspace*{0.1ex}\orientation{#1}\ifthenelse{\equal{#2}{}}{}{
%   \ifthenelse{\equal{#1}{}}{}{|}\body{#2}}%
%  }{ \hspace*{-0.2ex} \boldsymbol{R} }\vphantom{R}
%  } 

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Euler axis and angle: from orientation frame #1 belonging to body #2 to orientation frame #3 belonging to body #4, expressed in orientation frame #5
\newcommand{\eulerAxisAngle}[5]
 {\vphantom{e}_{\orientation{#5}}
 {\hspace*{-0.1ex}\boldsymbol{e}^{\orientation{#1}\ifthenelse{\equal{#2}{}}{}{|\body{#2}} ,\orientation{#3}\ifthenelse{\equal{#4}{}}{}{|\body{#4}}}}\vphantom{e}
 }
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Rotation vector: from orientation frame #1 belonging to body #2 to orientation frame #3 belonging to body #4, expressed in orientation frame #5
\newcommand{\rotationVector}[5]
 {\vphantom{r}_{\orientation{#5}}
 {\hspace*{-0.1ex}\boldsymbol{r}^{\orientation{#1}\ifthenelse{\equal{#2}{}}{}{|\body{#2}} ,\orientation{#3}\ifthenelse{\equal{#4}{}}{}{|\body{#4}}}}\vphantom{r}
 }
 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % symbol for euler angle rotation of orientation frame #1 on body #2 with respect to orientation frame #3 on body #4, with rotation around the axes #5 with angles #6
 \newcommand{\eulerAngleRot}[6]
 {
 \rot{#1}{#2}{#3}{#4}\left(\axis{#5} \ifthenelse{\equal{#6}{}}{}{}{,{#6}} \right)
 }
 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % symbol for RPY-angle rotation of orientation frame #1 on body #2 with respect to orientation frame #3 on body #4, with angles #5
 \newcommand{\RPYAngleRot}[5]
 {
 \rot{#1}{#2}{#3}{#4}\left(\axis{R}\axis{P}\axis{Y} \ifthenelse{\equal{#5}{}}{}{}{,{#5}} \right)
 }
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%s
  %symbol for quaternion from orientation frame #1 belonging to body #2 to orientation frame #3 belonging to body #4, expressed in orientation frame #5
 \newcommand{\quaternion}[5]
  {\vphantom{q}_{\orientation{#5}}
 {\hspace*{-0.1ex}\boldsymbol{q}^{\orientation{#1}\ifthenelse{\equal{#2}{}}{}{|\body{#2}} ,\orientation{#3}\ifthenelse{\equal{#4}{}}{}{|\body{#4}}}}\vphantom{q}
 }
 
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% POSE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% homogeneous transformation matrix, from frame {#1} fixed to body #2 to 
% frame {#2} fixed to body #4:
\newcommand{\htrans}[4]%
 {\vphantom{T}_{\refframe{#3}\ifthenelse{\equal{#4}{}}{}{|\body{#4}}}^{\hspace*{0.1ex}\refframe{#1}\ifthenelse{\equal{#2}{}}{}{|\body{#2}}}%
 {\hspace*{-0.1ex}\boldsymbol{T}}\vphantom{T}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%s
% finite displacement twist: pose of frame #1 fixed to body #2 wrt frame #3 fixed to body #4 
\newcommand{\finiteDisplacementTwist}[4]
{\vphantom{t}_{\refframe{#3}\ifthenelse{\equal{#4}{}}{}{|\body{#4}}}
^{\hspace*{0.1ex}\refframe{#1}\ifthenelse{\equal{#2}{}}{}{|\body{#2}}}
\textbf{\textsf{t}}_d 
\vphantom{\textbf{\textsf{t}}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%s
% screw axis: pose of frame #1 fixed to body #2 wrt frame #3 fixed to body #4 expressed in coordinate frame #5
\newcommand{\screwAxis}[5]
{\vphantom{SA}_{\orientation{#5}}
^{\hspace*{0.1ex}\refframe{#1}\ifthenelse{\equal{#2}{}}{}{|\body{#2}}}
\textbf{\textsf{SA}}_{\refframe{#3}\ifthenelse{\equal{#4}{}}{}{|\body{#4}}}
\vphantom{\textbf{\textsf{SA}}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TRANSLATIONAL VELOCITY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
 % translational velocity vector = derivative of position vector: from point #1 belonging to body #2 to point #3 belonging to body #4, expressed in orientation frame #5
\newcommand{\dposvec}[5]
 {
 \vphantom{p}_{\orientation{#5}}
 \hspace*{-0.1ex}\boldsymbol{\dot{p}}^{
 \ifthenelse{\equal{#1}{}}{
 {\ifthenelse{\equal{#2}{}}{}{\body{#2}} ,\point{#3}\ifthenelse{\equal{#4}{}}{}{|\body{#4}}}
 }
 {\forall\point{#1}\ifthenelse{\equal{#2}{}}{}{|\body{#2}} ,\point{#3}\ifthenelse{\equal{#4}{}}{}{|\body{#4}}}
 }
 \vphantom{p}
 }
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ROTATIONAL VELOCITY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% time derivative of rotation matrix:
\newcommand{\dotR}[4]%
  {\vphantom{R}_{\orientation{#3}\ifthenelse{\equal{#4}{}}{}{
  \ifthenelse{\equal{#3}{}}{}{|}
  \body{#4}}}^{\hspace*{0.1ex}\orientation{#1}\ifthenelse{\equal{#2}{}}{}{
  \ifthenelse{\equal{#1}{}}{}{|}\body{#2}}%
 }\dot{ \hspace*{-0.2ex} \boldsymbol{R} }\vphantom{R}
 } 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%s
% the rotational velocity vector of orientation frame #1 with respect to orientation frame #2, expressed in orientation frame #3
 \newcommand{\rotvec}[5]
 {\vphantom{ \boldsymbol{\omega} }^{
 \ifthenelse{\equal{#1}{}}{}{
\ifthenelse{\equal{#2}{}}{}{ \forall}}
 \orientation{#1}
 \ifthenelse{\equal{#1}{}}{}{
\ifthenelse{\equal{#2}{}}{}{ |}}
 \ifthenelse{\equal{#2}{}}{}{\body{#2}}}_{\orientation{#5}} \boldsymbol{\omega}_{
 \ifthenelse{\equal{#3}{}}{}{
 \ifthenelse{\equal{#4}{}}{}{\forall}}
  \orientation{#3}
  \ifthenelse{\equal{#3}{}}{}{
\ifthenelse{\equal{#4}{}}{}{ |}}
  \ifthenelse{\equal{#4}{}}{}{\body{#4}}}  \vphantom{ \boldsymbol{\omega} } }
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Euler angle rates of orientation frame #1 on body #2 with respect to orientation frame #3 on body #4, with rotation around the axes #5 with angles #6
\newcommand{\eulerAngleRates}[6]
 {
 \dotR{#1}{#2}{#3}{#4}\left(\axis{#5} \ifthenelse{\equal{#6}{}}{}{}{,{#6}} \right)
 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RPY angle rates of orientation frame #1 on body #2 with respect to orientation frame #3 on body #4, with rotation around the axes #5 with angles #6
\newcommand{\RPYAngleRates}[5]
 {
 \dotR{#1}{#2}{#3}{#4}\left(\axis{RPY} \ifthenelse{\equal{#5}{}}{}{}{,{#5}} \right)
 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%s
% quaternion rates from orientation frame #1 belonging to body #2 to orientation frame #3 belonging to body #4, expressed in orientation frame #5
\newcommand{\quaternionRates}[5]
  {\vphantom{q}_{\orientation{#5}}
 {\hspace*{-0.1ex}\boldsymbol{\dot{q}}^{\orientation{#1}\ifthenelse{\equal{#2}{}}{}{\ifthenelse{\equal{#1}{}}{}{|}\body{#2}} ,\orientation{#3}\ifthenelse{\equal{#4}{}}{}{\ifthenelse{\equal{#3}{}}{}{|}\body{#4}}}}\vphantom{q}
 }
 
  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TWIST
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%twist: velocity of point #1 belonging to body #2 with respect to body #3 expressed in orientation frame #4 (leave empty if not needed)
\newcommand{\twist}[4]
{
\vphantom{\textbf{\textsf{t}}}
^{ \point{#1}\hspace{0.1ex}|\hspace{0.1ex} \body{#2} }
_{\ifthenelse{\equal{#4}{}}{}{\orientation{#4}}}
\textbf{\textsf{t}}
_{\body{#3}}
\vphantom{\textbf{\textsf{t}}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%pose twist: pose twist of orientation frame #1 and point #1 belonging to body #2 wrt orientation frame #3 and point #3 belonging to body #3 
\newcommand{\posetwist}[4]
{
\vphantom{\textbf{\textsf{pt}}}
^{ \point{#1}\hspace{0.1ex}|\hspace{0.1ex} \body{#2} }
_{\ifthenelse{\equal{#4}{}}{}{\orientation{#4}}}
\textbf{\textsf{pt}}
_{\body{#3}}
\vphantom{\textbf{\textsf{pt}}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%screw twist: screw twist of orientation frame and point #2 belonging to body #1 wrt to body #3
\newcommand{\screwtwist}[3]
{
\vphantom{\textbf{\textsf{st}}}
^{ \point{#1}\hspace{0.1ex}|\hspace{0.1ex} \body{#2} }
_{\ifthenelse{\equal{#1}{}}{}{\orientation{#1}}}
\textbf{\textsf{st}}
_{\body{#3}}
\vphantom{\textbf{\textsf{st}}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%body-fixed twist: body fixed  twist of a orientation frame #1 and origin of #1 belonging to body #2 wrt body #3
\newcommand{\bodyfixedtwist}[3]
{
\vphantom{\textbf{\textsf{bt}}}
^{ \point{#1}\hspace{0.1ex}|\hspace{0.1ex} \body{#2} }
_{\ifthenelse{\equal{#1}{}}{}{\orientation{#1}}}
\textbf{\textsf{bt}}
_{\body{#3}}
\vphantom{\textbf{\textsf{bt}}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% homogeneous transformation matrix derivative, from point {#1} fixed to body #2 to 
% wrt body #4 expressed in orientation frame #3:
\newcommand{\dothtrans}[4]%
 {\vphantom{T}_{\orientation{#3}\ifthenelse{\equal{#4}{}}{}{|\body{#4}}}^{\hspace*{0.1ex}\point{#1}\ifthenelse{\equal{#2}{}}{}{|\body{#2}}}%
 {\hspace*{-0.1ex}\dot{\boldsymbol{T}}}\vphantom{T}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%s
% instantaneous screw axis: velocity of body #1 wrt body #2 expressed in coordinate frame #3
\newcommand{\instantaneousScrewAxis}[3]
{\vphantom{ISA}_{\orientation{#3}}
^{\hspace*{0.1ex}\ifthenelse{\equal{#1}{}}{}{\body{#1}}}
\textbf{\textsf{ISA}}_{\body{#2}}
\vphantom{\textbf{\textsf{ISA}}}
}

==> macroOperations.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% change ref point from point #1 on body#3 to point #2 on body#3, expressed in frame #4  (for the body of which position is expressed)
\newcommand{\changeRefPointBody}[4]
 {\vphantom{\boldsymbol{M}}_{
 \ifthenelse{\equal{#4}{}}{}{ \orientation{#4}} }
 \hspace*{-0.3ex} \boldsymbol{M}_{\textrm{body}}^{\point{#1}
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } 
, \point{#2} 
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } }
\vphantom{\boldsymbol{M}}}

% change ref point from point #1 on body#3 to point #2 on body#3, expressed in frame #4 (for reference body)
\newcommand{\changeRefPointRefBody}[4]
 {\vphantom{\boldsymbol{M}}_{
 \ifthenelse{\equal{#4}{}}{}{ \orientation{#4}} }
 \hspace*{-0.3ex} \boldsymbol{M}_{\textrm{ref}}^{\point{#1}
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } 
, \point{#2} 
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } }
\vphantom{\boldsymbol{M}}}


% change ref frame from orientation frame #1 to orientation frame #2 
\newcommand{\changeRefFrame}[2]
 {\vphantom{\boldsymbol{P}}_{\orientation{#2}}^{\orientation{#1}}
  \hspace*{-0.3ex} \boldsymbol{P} \vphantom{\boldsymbol{N}} \hspace{0.3ex}}

% change orientation frame from orientation frame #1 on body#3 to orientation frame #2 on body#3, expressed in frame #4 (for the body of which orientation is expressed)
\newcommand{\changeOrientationFrameBody}[4]
 {\vphantom{\boldsymbol{N}}_{
 \ifthenelse{\equal{#4}{}}{}{ \orientation{#4}} }
 \hspace*{-0.3ex} \boldsymbol{N}_{\textrm{body}}^{\orientation{#1}
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } 
, \orientation{#2} 
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } }
\vphantom{\boldsymbol{N}}}

% change frame from frame #1 on body#3 to  frame #2 on body#3, expressed in frame #4 (for the body of which orientation is expressed)
\newcommand{\changeFrameBody}[4]
 {\vphantom{\boldsymbol{S}}_{
 \ifthenelse{\equal{#4}{}}{}{ \orientation{#4}} }
 \hspace*{-0.3ex} \boldsymbol{S}_{\textrm{body}}^{\refframe{#1}
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } 
, \refframe{#2} 
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } }
\vphantom{\boldsymbol{S}}}

% change frame from frame #1 on body#3 to  frame #2 on body#3, expressed in frame #4 (for the reference body)
\newcommand{\changeFrameRefBody}[4]
 {\vphantom{\boldsymbol{S}}_{
 \ifthenelse{\equal{#4}{}}{}{ \orientation{#4}} }
 \hspace*{-0.3ex} \boldsymbol{S}_{\textrm{ref}}^{\refframe{#1}
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } 
, \refframe{#2} 
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } }
\vphantom{\boldsymbol{S}}}


% change orientation frame from orientation frame #1 on body#3 to orientation frame #2 on body#3, expressed in frame #4 (for reference body)
\newcommand{\changeOrientationFrameRefBody}[4]
 {\vphantom{\boldsymbol{N}}_{
 \ifthenelse{\equal{#4}{}}{}{ \orientation{#4}} }
 \hspace*{-0.3ex} \boldsymbol{N}_{\textrm{ref}}^{\orientation{#1}
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } 
, \orientation{#2} 
\ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } }
\vphantom{\boldsymbol{N}}}

% change ref point and reference frame together from #1 to #2 of reference body
\newcommand{\changeRefPointOrientationFrameRefBody}[3]
 {\vphantom{\boldsymbol{S}}_{\refframe{#2}
 \ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} }
 }^{\refframe{#1}
 \ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} }
 }
  \hspace*{-0.3ex} \boldsymbol{S}_{\textrm{ref}} \vphantom{\boldsymbol{S}}
  \hspace{0.7ex}
  }
  
  % change ref point and reference frame together from #1 to #2 of body
\newcommand{\changeRefPointOrientationFrameBody}[3]
 {\vphantom{\boldsymbol{S}}_{\refframe{#2}
 \ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} }
 }^{\refframe{#1}
 \ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} }
 }
  \hspace*{-0.3ex} \boldsymbol{S}_{\textrm{body}} \vphantom{\boldsymbol{S}}
  \hspace{0.7ex}
  }
  
% change ref point and reference frame + frame in which expressed together from #1 to #2 fixed to body #3
\newcommand{\changeRefFrameRefBody}[3]
 {\vphantom{\boldsymbol{S}}_{\refframe{#2}
 \ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } 
 }^{
 \refframe{#1}
 \ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } 
 }
  \hspace*{-0.3ex} \boldsymbol{S} \vphantom{\boldsymbol{S}}
  \hspace{0.7ex}
  }  

% change ref point and orientation frame in which projected
\newcommand{\changeRefPointBodyRefFrame}[3]
 {\vphantom{\boldsymbol{S}}_{\refframe{#2}
 \ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} }
 }^{
 \refframe{#1}
 \ifthenelse{\equal{#3}{}}{}{\hspace{0.1ex}|\hspace{0.3ex} \body{#3} } 
 }
  \hspace*{-0.3ex} \boldsymbol{S} \vphantom{\boldsymbol{S}}
  \hspace{0.7ex}
  }  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\composePosition}[2]
{#1 + #2 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\composeOrientation}[2]
{#1 + #2 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\composePose}[2]
{#1 + #2 }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\composeTranslationVelocity}[2]
{#1 + #2 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\composeRotationVelocity}[2]
{#1 + #2 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\composeVelocity}[2]
{#1 + #2 }
